Controlling Directions Orthogonal to a Classifier

We propose to identify directions invariant to a given classifier so that these directions can be controlled in tasks such as style transfer. While orthogonal decomposition is directly identifiable when the given classifier is linear, we formally define a notion of orthogonality in the non-linear case. We also provide a surprisingly simple method for constructing the orthogonal classifier (a classifier utilizing directions other than those of the given classifier). Empirically, we present three use cases where controlling orthogonal variation is important: style transfer, domain adaptation, and fairness. The orthogonal classifier enables desired style transfer when domains vary in multiple aspects, improves domain adaptation with label shifts and mitigates the unfairness as a predictor. The code is available at http://github.com/Newbeeer/orthogonal_classifier

==> dump.tex <==
% We are often interested in learning an energy function of $p(\vx)$, i.e. some $f(\vx) = \log p(\vx) + C$, which is parametrized by $\theta$, denoted as $f_\theta(\vx)$. Let us consider the log density ratio quantity:
% \begin{align}
%     r_{\theta, \phi}(\vx) = \log \frac{p_\theta(\vx)}{q_\phi(\vx)}
% \end{align}
% where $p_\theta(\vx) \propto \exp(f_\theta(\vx))$ is the distribution derived from our energy and $q_\phi(\vx)$ is some ``initial proposal distribution''. It is obvious that:
% \begin{align}
%     f_\theta(\vx) = r_{\theta, \phi}(\vx) + q_\phi(\vx) + C
% \end{align}
% To remove the need of learning a partition function of $f_\theta$, we instead reparametrize $r_{\theta, \phi}(\vx)$ as $r_{\psi}(\vx)$, and our energy function would then become
% \begin{align}
%     f_{\psi}(\vx) = r_{\psi}(\vx) + q_\phi(\vx) + C
% \end{align}

% Let us now consider some f-divergence between the distribution of $\pdata$ and $q_\phi$.
% \begin{align*}
%     D_{f}(\pdata(\vx) \Vert q_\phi(\vx)) = \max_\psi (\bb{E}_{\vx \sim \pdata(\vx)}[f'(\exp(r_{\psi}(\vx)))] - \bb{E}_{\vx \sim q(\vx)}[f^\star(f'(\exp(r_{\psi}(\vx))))])
% \end{align*}
% We note that the optimal solution for $r_{\psi, \phi}$ is $\log \pdata(\vx) - \log q_\phi(\vx)$.

% \begin{gather}
%     f(u) = u \log u - (u+1) \log (u+1) \\
%     f^\star(v) = - \log (1 - \exp(v)) \\
%     f'(u) = \log u - \log (u+1)
% \end{gather}
% and
% \begin{gather}
%     f' \circ \exp (r) = r - \log (\exp(r) + 1) \\
%     f^\star \circ f' \circ \exp(r) = - \log (\exp(r) + 1)
% \end{gather}
% which allows us to recover NCE.

\section{KL Divergence}
Unfortunately, the argument does not work well for KL-divergences because the Nyugen's bound is too loose. A tighter version of the bound gives rise to the Donsker-Valadahn's inequality. Consider this for $\pdata(\vx)$ and $q_\phi(\vx)$
\begin{align}
    \min_\phi D_{\mathrm{KL}}(\pdata \Vert q_\phi) = \min_\phi \max_\psi (\bb{E}_{\vx \sim \pdata(\vx)}[r_{\psi}(\vx)] - \log \bb{E}_{\vx \sim q(\vx)}[\exp(r_{\psi}(\vx))])
\end{align}
We note that the maximum is again obtained at $r_{\psi}(\vx) = \log \pdata - \log q_\phi$. We can reformulate this to the adversarial dynamics embedding objective by noting that:
\begin{align}
    \log \bb{E}_{\vx \sim q_\phi(\vx)}[\exp(r_{\psi}(\vx))]) & \geq \bb{E}_{\vx \sim q(\vx)}[r_{\psi}(\vx)] \\
    & = \bb{E}_{\vx \sim q(\vx)}[(r_{\psi}(\vx) + \log q_\phi(\vx)) - \log q_\phi(\vx)] \\
    & = \bb{E}_{\vx \sim q(\vx)}[f_{\psi, \phi}(\vx) - \log q_\phi(\vx)]
\end{align}
where the last objective highlights the fact that our intended energy based model is $f_{\psi, \phi}(\vx) = r_\psi(\vx) + \log q_\phi(\vx)$.

So by fixing $r_\psi$, we maximize $\bb{E}_{\vx \sim q(\vx)}[r_{\psi}(\vx)]$ to obtain $\log \bb{E}_{\vx \sim q_\phi(\vx)}[\exp(r_{\psi}(\vx))])$.

Then 
\begin{align}
    \min_\phi D_{\mathrm{KL}}(\pdata \Vert q_\phi) &= \min_\phi \max_\psi (\bb{E}_{\vx \sim \pdata(\vx)}[r_{\psi}(\vx)] - \log \bb{E}_{\vx \sim q(\vx)}[\exp(r_{\psi}(\vx))]) \\
    & \leq \min_\phi \max_\psi  (\bb{E}_{\vx \sim \pdata(\vx)}[r_{\psi}(\vx)] - \bb{E}_{\vx \sim q(\vx)}[r_{\psi}(\vx)]) \\
    & = \min_\phi \max_\psi  (\bb{E}_{\vx \sim \pdata(\vx)}[f_{\psi, \phi}(\vx) - \log q_\phi(\vx)] - \bb{E}_{\vx \sim q(\vx)}[f_{\psi, \phi}(\vx) - \log q_\phi(\vx)]) \\
    & = \min_\phi \max_\psi  \underbrace{(\bb{E}_{\vx \sim \pdata(\vx)}[f_{\psi, \phi}(\vx)] - \bb{E}_{\vx \sim q(\vx)}[f_{\psi, \phi}(\vx)] - H(q_\phi))}_{\text{Dual objective of ADE}} - \underbrace{\bb{E}_{\vx \sim \pdata(\vx)}[\log q_\phi(\vx)]}_{\text{Maximum Likelihood of $q_\phi$}}
\end{align}
Where the ADE objective~\citep{dai2019exponential} simply uses the dual formulation of the log partition function~\citep{wainwright2008graphical}:
\begin{align}
    \max_\psi \min_\phi  \bb{E}_{\vx \sim \pdata(\vx)}[f_{\psi, \phi}(\vx)] - \bb{E}_{\vx \sim q(\vx)}[f_{\psi, \phi}(\vx)] - H(q_\phi)
\end{align}

\section{Person's $\chi^2$ divergence}
We can also derive a close form for the tight bound for $\chi^2$-divergence, where
\begin{align}
    (I^R_{f, q})^\star(T) = \int (\frac{T^2}{4} + T) \mathrm{d} q - \frac{(\int T \mathrm{d} q)^2}{4}
\end{align}
Therefore, 
\begin{align}
    D_{\chi^2}(\pdata \Vert q_\phi) & \geq 2\bb{E}_{\pdata}[\exp(r_{\psi}(\vx)) - 1] - 2\bb{E}_{q_\phi}[\exp(r_{\psi}(\vx)) - 1] - \bb{E}_{q_\phi}[(\exp(r_{\psi}(\vx)) - 1)^2] + (\bb{E}_{q_\phi}[\exp(r_{\psi}(\vx)) - 1])^2 %\\
    % & = 2\bb{E}_{\pdata}[\exp(r_{\psi}(\vx)) - 1] - \bb{E}_{q_\phi}[\exp(r_{\psi}(\vx))^2] - 1 + (\bb{E}_{q_\phi}[\exp(r_{\psi}(\vx)) - 1])^2
\end{align}
Since $g(u) = u^2$ is convex, we have:
\begin{align}
    (\bb{E}_{q_\phi}[\exp(r_{\psi}(\vx)) - 1])^2 \leq \bb{E}_{q_\phi}[(\exp(r_{\psi}(\vx)) - 1)^2]
\end{align}
Then we can obtain the following minimax objective:
\begin{align*}
    & \min_{\phi} \max_{\psi} D_{\chi^2}(\pdata \Vert q_\phi) \\
    = &  \min_{\phi} \max_{\psi} 2\bb{E}_{\pdata}[\exp(r_{\psi}(\vx)) - 1] - 2\bb{E}_{q_\phi}[\exp(r_{\psi}(\vx)) - 1] - \bb{E}_{q_\phi}[(\exp(r_{\psi}(\vx)) - 1)^2] + (\bb{E}_{q_\phi}[\exp(r_{\psi}(\vx)) - 1])^2 \\
    % = &  \max_{\psi} \min_{\phi} 2\bb{E}_{\pdata}[\exp(r_{\psi}(\vx)) - 1] - 2\bb{E}_{q_\phi}[\exp(r_{\psi}(\vx)) - 1] - \bb{E}_{q_\phi}[(\exp(r_{\psi}(\vx)) - 1)^2] + (\bb{E}_{q_\phi}[\exp(r_{\psi}(\vx)) - 1])^2 \\
    \leq & \min_{\phi} \max_{\psi}  2\bb{E}_{\pdata}[\exp(r_{\psi}(\vx)) - 1] - 2\bb{E}_{q_\phi}[\exp(r_{\psi}(\vx)) - 1] - \bb{E}_{q_\phi}[(\exp(r_{\psi}(\vx)) - 1)^2] + \bb{E}_{q_\phi}[(\exp(r_{\psi}(\vx)) - 1)^2] \\
    = & \min_{\phi} \max_{\psi} 2\bb{E}_{\pdata}[\exp(r_{\psi}(\vx)) - 1] - 2\bb{E}_{q_\phi}[\exp(r_{\psi}(\vx)) - 1]
\end{align*}

\section{General Minimax Objectives}

From the Pearson and KL examples we find that both objectives have the following form:
\begin{align}
    \min_\phi \max_\psi \bb{E}_{\pdata(\vx)}[f'(\exp(r_\psi(\vx))] - \bb{E}_{q_\phi(\vx)}[f'(\exp(r_\psi(\vx))]
\end{align}
To see this, note that $f'(u) = \log u + 1$ for KL, and $f'(u) = 2 u$ for Pearson.
There is a saddle point where $q_\phi = \pdata$ and $r_\psi = C$. \js{We can make $r_\psi = 0$ wlog.}

The following minimax objective also has a saddle point such that $q_\phi = \pdata$ and $r_\psi = C$:
\begin{align}
    \min_\phi \max_\psi \bb{E}_{\pdata(\vx)}[f'(\exp(r_\psi(\vx))] - \bb{E}_{q_\phi(\vx)}[f^\star(f'(\exp(r_\psi(\vx)))]
\end{align}
which is based on the NWJ lower bound on $f$-divergence.

In fact, they can be connected by the following inequality:
\begin{align}
\bb{E}_{\pdata(\vx)}[f'(\exp(r_\psi(\vx))] - \bb{E}_{q_\phi(\vx)}[f'(\exp(r_\psi(\vx))] 
   \geq \bb{E}_{\pdata(\vx)}[f'(\exp(r_\psi(\vx))] - \bb{E}_{q_\phi(\vx)}[f^\star(f'(\exp(r_\psi(\vx)))]
\end{align}
To see why this true, simply apply the definition of Fenchel duality:
\begin{align}
    f^\star(u) \geq u - f(1)
\end{align}
where $f(1) = 0$ by assumption over f-divergences. The equality holds when $r_\psi(\vx) = 0$ everywhere.

Therefore, we summarize two general minimax objectives based on f-divergences.

\paragraph{f-Contrastive Divergence}
\begin{align}
    \min_\phi \max_\psi \bb{E}_{\pdata(\vx)}[f'(\exp(r_\psi(\vx))] - \bb{E}_{q_\phi(\vx)}[f'(\exp(r_\psi(\vx))]
\end{align}
This form contains the ADE method, the proposed Pearson minimax objective and CD. 

\paragraph{NWJ Variational Bounds}
\begin{align}
\min_\phi \max_\psi \bb{E}_{\pdata(\vx)}[f'(\exp(r_\psi(\vx))] - \bb{E}_{q_\phi(\vx)}[f^\star(f'(\exp(r_\psi(\vx)))]
\end{align}
This form contains the NCE method. 

Again, we note that the energy function we learn is $r_\psi(\vx) + \log q_\phi(\vx)$, but we are free to choose to formulate the objective with the energy function directly.

% \section{Outline}

% \begin{itemize}
%     \item There exists general bounds on $f$-divergences where the optimal variational approximation is obtained as a function of density ratios.
%     \item Give a ``proposal distribution'' with tractable density, we can obtain suitable objective to training energy-based models under $f$-divergences.
%     \item We show that this contains related existing objectives, such as NCE.
%     \item This generalization allows us to propose new objectives to learning energy based models (e.g. the new bound with Pearson $\chi^2$ divergences)
%     \item From the Pearson example, we summarize two simple families of objectives which can be applied with any f-divergence. The two families of objectives include ones that have been proposed.
% \end{itemize}

% \paragraph{f-Contrastive Divergence}
% \begin{align}
%     \min_\phi \max_\psi \bb{E}_{\pdata(\vx)}[f'(\exp(r_\psi(\vx))] - \bb{E}_{q_\phi(\vx)}[f'(\exp(r_\psi(\vx))]
% \end{align}
% This form contains the ADE method, the proposed Pearson minimax objective and CD. 

% \paragraph{NWJ Variational Bounds}
% \begin{align}
% \min_\phi \max_\psi \bb{E}_{\pdata(\vx)}[f'(\exp(r_\psi(\vx))] - \bb{E}_{q_\phi(\vx)}[f^\star(f'(\exp(r_\psi(\vx)))]
% \end{align}
% This form contains the NCE method. 

% \section{Two Types of Bounds based on Fenchel Duality}
% There is a tighter bound for $f$-divergences than the one proposed by NWJ:
% \begin{align}
%      D_{f}(p(\vx) \Vert q(\vx)) \geq \bb{E}_{\vx \sim p(\vx)}[T(\vx)] - 
%      (I^R_{f, q})^\star(T) \geq \bb{E}_{\vx \sim p(\vx)}[T(\vx)] - 
%      \bb{E}_q[f^\star(T)]
% \end{align}
% where $I^R_{f, q}(r) = \bb{E}_{\vx \sim q(\vx)}[f(r(\vx))]$ where $r \in \Delta(q)$, which means $\int r \mathrm{d} q = 1$. For example, the probability ratio between $p$ and $q$ is a member of $\Delta(q)$. $(I^R_{f, q})^\star$ is the Fenchal dual of $I^R_{f, q}$:
% \begin{align}
%     (I^R_{f, q})^\star(T) = \sup_{r \in \Delta(q)} \left\{ \bb{E}_{q}[T r] - I_{f, q}^R(r) \right\}
% \end{align}
% The DV inequality is an instance of the tighter bound.


\section{Background}
We consider data samples denoted as $\vx$ from the set $\gX$. Given a dataset with empirical distribution $\pdata(\vx)$, we are interested in learning an (unnormalized) energy function $E_\theta(\vx)$ that prescribes the following normalized distribution:
\begin{align}
    p_\theta(\vx) = \frac{e^{-E_\theta(\vx)}}{Z_{\theta}}
\end{align}
where
\begin{align}
    Z_\theta = \int e^{-E_\theta(\vx)} \mathrm{d} \vx
\end{align}
is a normalization constant (called the partition function).

\subsection{Contrastive Divergence}
The maximum likelihood solution for $p_\theta(\vx)$ is given by minimizing the following objective:
\begin{align}
    \gL_{\mathrm{MLE}}(\theta; \pdata) \defeq -\bb{E}_{\vx \sim \pdata(\vx)}\left[\log p_\theta(\vx)\right]
\end{align}
whose gradient is equivalent to
\begin{align}
    \nabla_\theta \gL_{\mathrm{MLE}}(\theta; \pdata) & = \nabla_\theta \bb{E}_{\vx \sim \pdata(\vx)}\left[-\log p_\theta(\vx)\right] \\
    & = \nabla_\theta \bb{E}_{\vx \sim \pdata(\vx)}[E_\theta(\vx)] + \nabla_\theta \log Z_\theta \\
    & = \nabla_\theta \bb{E}_{\vx \sim \pdata(\vx)}[E_\theta(\vx)] - \frac{\int e^{-E_\theta(\vx)} \nabla_\theta E_\theta(\vx) \mathrm{d} \vx}{Z_\theta} \\
    & = \nabla_\theta \left(\bb{E}_{\vx \sim \pdata(\vx)}[E_\theta(\vx)] - \bb{E}_{\vx \sim p_\theta(\vx)}[E_\theta(\vx)]\right)
\end{align}
This gives rise to the Constrastive Divergence (CD) objective:
\begin{align}
    \gL_{\mathrm{CD}}(\theta; \pdata) = \bb{E}_{\vx \sim \pdata(\vx)}[E_\theta(\vx)] - \bb{E}_{\vx \sim p_\theta(\vx)}[E_\theta(\vx)]
\end{align}
which is equivalent to MLE (up to a constant). Intuitively this amounts to decreasing the energy of ``positive'' samples (from $\pdata$) and increasing the energy of ``negative samples'' (from $p_\theta$)

MCMC techniques are needed in order to sample from $p_\theta(\vx)$, which is undesirable when the MCMC chain converges slowly to the stationary distribution.

\subsection{Dual formulation of Maximum Likelihood}
As an alternative to CD, one could consider the Frenchal dual of the log-partition function~\citep{wainwright2008graphical,dai2019exponential}.

\begin{lemma} Let $H(q) = \bb{E}_{\vx \sim q}[-\log q]$ denote the entropy of $q$, we have
\begin{align}
    \log Z_\theta = \max_{q \in \gP(\gX)} \bb{E}_{\vx \sim q(\vx)}[-E_\theta(\vx)] + H(q)
\end{align}
and the maximum is obtained when $q(\vx) \propto e^{-E_\theta(\vx)}$.
\end{lemma}
\begin{proof}
\begin{align}
    & \ \bb{E}_{\vx \sim q(\vx)}[-E_\theta(\vx)] - H(q) \\
     = & \ \bb{E}_{\vx \sim q(\vx)}[-E_\theta(\vx) - \log q(\vx)] = \bb{E}_{\vx \sim q(\vx)}\left[\log \frac{e^{-E_\theta(\vx)}}{q(\vx)}\right] \\
    \leq & \ \log \bb{E}_{\vx \sim q(\vx)}\left[ \frac{e^{-E_\theta(\vx)}}{q(\vx)}\right] = \log Z_\theta
\end{align}
\end{proof}

Therefore, we can rewrite $\log p_\theta$ as 
\begin{align}
    \bb{E}_{\vx \sim \pdata(\vx)}\log p_\theta(\vx) & = \bb{E}_{\vx \sim \pdata(\vx)}[-E_\theta(\vx)] - \max_{q \in \gP(\gX)} \left(\bb{E}_{\vx \sim q(\vx)}[-E_\theta(\vx)] + H(q)\right) \\
    & = \min_{q \in \gP(\gX)} \bb{E}_{\vx \sim \pdata(\vx)}[-E_\theta(\vx)] + \bb{E}_{\vx \sim q(\vx)}[E_\theta(\vx)] - H(q)
\end{align}
This leads to the following minimax objective when we parametrize $q(\vx)$ with $\phi$:
\begin{gather}
    \min_\theta \max_\phi \gL_{\mathrm{MLE-D}}(\theta, \phi; \pdata) \\
    \mathrm{where } \quad \gL_{\mathrm{MLE-D}}(\theta, \phi; \pdata) = \bb{E}_{\vx \sim q(\vx)}[E_\theta(\vx)] - \bb{E}_{\vx \sim \pdata(\vx)}[E_\theta(\vx)] + H(q)
\end{gather}
which we use MLE-D to denotes the usage of a dual formulation. Here, we no longer require samples from $p_\theta$, but require a dual model $q_\phi(\vx)$ that has tractable sampling procedure and tractable likelihood.

\subsection{Noise Contrastive Estimation}
The noise contrastive estimation objective considers an alternative approach to maximum likelihood by selecting a reference (noise) distribution $q(\vx)$:
\begin{gather}
 \max_\theta \gL_{\mathrm{NCE}}(\theta; \pdata, q) \\
   \mathrm{where } \quad \gL_{\mathrm{NCE}}(\theta; \pdata, q) = \E_{\pdata}\left[\log \frac{e^{-E_\theta(\vx)}}{e^{-E_\theta(\vx)} + q(\vx)}\right] + \E_{q(\vx)}\left[\log \frac{q(\vx)}{e^{-E_\theta(\vx)} + q(\vx)}\right]
\end{gather}

\subsection{Variational bounds on $f$-divergences for likelihood ratio estimation}

Maximum likelihood of $p_\theta$ over $\pdata$ is equivalent to minimizing the KL divergence $D_{\mathrm{KL}}(\pdata \Vert p_\theta)$, which motivates learning an energy function in terms of divergence minimization. Moreover, KL divergences belong to a family of $f$-divergences:
\begin{align}
    D_{f}(p(\vx) \Vert q(\vx)) = \bb{E}_{\vx \sim q(\vx)}\left[f\left(\frac{p(\vx)}{q(\vx)}\right)\right]
\end{align}
where the generator function $f: \R^+ \to \R$ is a convex, lower-semicontinuous function satisfying $f(1) = 0$. There is a lower bound on the divergence:
\begin{align}
    D_{f}(p(\vx) \Vert q(\vx)) = \sup_{T}(\bb{E}_{\vx \sim p(\vx)}[T(\vx)] - \bb{E}_{\vx \sim q(\vx)}[f^\star(T(\vx))])
\end{align}
where $T$ belongs to an arbitrary function $T: \gX \to \R$. This bound is tight for 
\begin{align}
T^\star(\vx) = f'\left(\frac{p(\vx)}{q(\vx)} \right) 
\end{align}
which can be shown from the definition of convex conjugate.

\subsection{Tighter duality bounds on $f$-divergences}
Denote $I_{f, q}(r) = \bb{E}_{\vx \sim q(\vx)}[f(r(\vx))]$, and the $f$-divergence between $p(\vx)$ and $q(\vx)$ is recovered by setting $r = p/q$:
\begin{align}
    D_{f}(p(\vx) \Vert q(\vx)) = \bb{E}_{\vx \sim q(\vx)}\left[f\left(\frac{p(\vx)}{q(\vx)}\right)\right] = I_{f, q}(p/q)
\end{align}
We denote $r \in \Delta(q)$ if and only if $\int r \mathrm{d} q = 1$. For example, $p / q$ is a member of $\Delta(q)$. From the definition of convex conjugate, we have the following lemma~\citep{ruderman2012tighter}.

\begin{lemma}
Define
\begin{align}
    (I_{f, q})^\star(T) = \sup_{r \in \Delta(q)} \left\{ \bb{E}_{q}[T r] - I_{f,q}(r) \right\}
\end{align}
then for all $T$ \js{quantifier}
\begin{align}
     D_{f}(p(\vx) \Vert q(\vx)) \geq \bb{E}_{\vx \sim p(\vx)}[T(\vx)] - 
     (I_{f, q})^\star(T) \geq  \bb{E}_{\vx \sim p(\vx)}[T(\vx)] - \bb{E}_q[f^\star(T)]
\end{align}
where equality is obtained when $T(\vx) = f'\left(\frac{p(\vx)}{q(\vx)}\right)$.
\end{lemma}

The above lemma shows that a tighter variational lower bound could be found by restricting the space of $r$. An interesting application of this lemma is over the KL divergence:
\begin{corollary}[Donsker-Valadahn Inequality]

\end{corollary}
\begin{proof}
Directly apply $f$ to KL and consider the functional derivative of $(I_{f, q})^\star(T)$.
\end{proof}

% There is a tighter bound for $f$-divergences than the one proposed by NWJ:
% \begin{align}
%      D_{f}(p(\vx) \Vert q(\vx)) \geq \bb{E}_{\vx \sim p(\vx)}[T(\vx)] - 
%      (I^R_{f, q})^\star(T) \geq \bb{E}_{\vx \sim p(\vx)}[T(\vx)] - 
%      \bb{E}_q[f^\star(T)]
% \end{align}
% where $I^R_{f, q}(r) = \bb{E}_{\vx \sim q(\vx)}[f(r(\vx))]$ where $r \in \Delta(q)$, which means $\int r \mathrm{d} q = 1$. For example, the probability ratio between $p$ and $q$ is a member of $\Delta(q)$. $(I^R_{f, q})^\star$ is the Fenchal dual of $I^R_{f, q}$:
% \begin{align}
%     (I^R_{f, q})^\star(T) = \sup_{r \in \Delta(q)} \left\{ \bb{E}_{q}[T r] - I_{f, q}^R(r) \right\}
% \end{align}
% The DV inequality is an instance of the tighter bound.

\subsection{Integral Probability Metrics}
\js{todo} For a particular class $gF$ of functions $f: \gX \to \bb{R}$, then 
\begin{align}
    \rho_{\gF}(p \Vert q) = \sup_{T \in \gF} \Big|\bb{E}_{\vx \sim p(\vx)}[T(\vx)] - \bb{E}_{\vx \sim q(\vx)}[T(\vx)]\Big|
\end{align}

\section{Learning Energy-based Models with $f$-Contrastive Divergence}
In this section, we consider two formulations of parametrizing the energy function. One is to use $E_\theta$ directly; another is to consider the energy to be the sum of two components:
\begin{enumerate}
    \item Log-likelihood of proposal model $\log q_\phi(\vx)$, where $q_\phi(\vx)$ is a likelihood-based generative model of $\vx$ with tractable densities and tractably sampling.
    \item Residual model $r_\psi(\vx)$, which models the difference between the negative energy and the proposal log-likelihood.
\end{enumerate}
In this case, the energy function is modeled via $ -\log q_\phi(\vx) - r_\psi(\vx)$.

\subsection{$f$-Constrastive Divergence}
We first present the $f$-Contrastive Divergence ($f$-CD) objective under the second formulation (with $\log q_\phi$ and $r$). For any valid choice of convex semi-continuous $f: \bb{R} \to \bb{R}$ with $f(1) = 0$, we have the following objective:
\begin{gather}
 \min_\phi \max_\psi \gL_{f-\mathrm{CD}2}(\psi, \phi; \pdata) \\
    \mathrm{where } \quad \gL_{f-\mathrm{CD}1}(\psi, \phi; \pdata) = \bb{E}_{\pdata(\vx)}[f'(\exp(r_\psi(\vx))] - \bb{E}_{q_\phi(\vx)}[f'(\exp(r_\psi(\vx))]
\end{gather}
Equivalently, if we consider representing the energy with $-E_\theta(\vx)$ directly, then this objective is be written as
\begin{gather}
    \min_\phi \max_\theta \gL_{f-\mathrm{CD}1}(\theta, \phi; \pdata) \\
    \mathrm{where } \quad \gL_{f-\mathrm{CD}2}(\theta, \phi; \pdata) = \bb{E}_{\pdata(\vx)}[f'(e^{-E_\theta(\vx) - \log q_\phi(\vx)})] - \bb{E}_{q_\phi(\vx)}[f'(e^{-E_\theta(\vx) - \log q_\phi(\vx)})] \nonumber
\end{gather}

\paragraph{Connection with Contrastive Divergence} In CD, we consider a fixed MCMC approach to obtain samples that only depends on the energy function $E_\theta(\vx)$. Under KL divergence $f'(\exp(u)) = u + 1$, so 
\begin{align}
    \gL_{f-\mathrm{CD}2}(\psi, \phi; \pdata) &= \bb{E}_{\pdata(\vx)}[-E_\theta(\vx) - \log q_\phi(\vx)] - \bb{E}_{q_\phi(\vx)}[-E_\theta(\vx) - \log q_\phi(\vx))] \\
    & = - (\bb{E}_{\pdata(\vx)}[E_\theta(\vx)] - \bb{E}_{q_\phi(\vx)}[E_\theta(\vx)]) - (\bb{E}_{\pdata(\vx)}[\log q_\phi(\vx)] - \bb{E}_{q_\phi(\vx)}[\log q_\phi(\vx)]) \nonumber
\end{align}
where the second part of the last term is ignored when we optimize for $\theta$ (due to non-continuity of MCMC sampling).

\paragraph{Connection with Maximum-likelihood Dual form}
Rearranging terms, we have
\begin{align}
    \gL_{f-\mathrm{CD}2}(\psi, \phi; \pdata) &= \bb{E}_{\pdata(\vx)}[-E_\theta(\vx) - \log q_\phi(\vx)] - \bb{E}_{q_\phi(\vx)}[-E_\theta(\vx) - \log q_\phi(\vx))] \\
    & = - (\bb{E}_{\pdata(\vx)}[E_\theta(\vx)] - \bb{E}_{q_\phi(\vx)}[E_\theta(\vx)]) - (\bb{E}_{\pdata(\vx)}[\log q_\phi(\vx)] - \bb{E}_{q_\phi(\vx)}[\log q_\phi(\vx)]) \nonumber \\
    & = \underbrace{-\bb{E}_{\pdata(\vx)}[E_\theta(\vx)] - \bb{E}_{q_\phi(\vx)}[E_\theta(\vx)] - H(q_\phi)}_{\gL_{\mathrm{MLE-D}}} - \bb{E}_{\pdata(\vx)}[\log q_\phi(\vx)]
\end{align}
The last term is the maximum likelihood solution of $q_\phi(\vx)$ under $\pdata(\vx)$ which coincides with the case the lower bound $\gL_{\mathrm{MLE-D}}$ is tight.

\subsection{$f$-CD as Variational $f$-Divergence Minimization}
The following variational lower bound for $f$-divergence:
\begin{align}
     \bb{E}_{\vx \sim p(\vx)}[T(\vx)] - 
     (I_{f, q})^\star(T) \leq D_{f}(p(\vx) \Vert q(\vx))
\end{align}
can also be interpreted as a lower bound of $\gL_{f-\mathrm{CD}2}$.
\begin{proposition}
For all $T$, $p(\vx)$, $q(\vx)$ \js{quantifiers}, we have
\begin{align}
    \bb{E}_{\vx \sim p(\vx)}[T(\vx)] - 
     (I_{f, q})^\star(T) \leq \bb{E}_{\vx \sim p(\vx)}[T(\vx)] - \bb{E}_{\vx \sim q(\vx)}[T(\vx)]
\end{align}
where $(I_{f, q})^\star(T)$ is defined in \js{lemma}.
\end{proposition}
\begin{proof}
Let $r(\vx) = 1$ for all $\vx \in \gX$, then
\begin{align}
 \bb{E}_{\vx \sim q(\vx)}[T(\vx)] = \bb{E}_q[T(\vx) r(\vx)] = \bb{E}_q[T(\vx) r(\vx)] - I_{f, q}(r)
    \leq \sup_{r \in \Delta(q)}\{\bb{E}_q[Tr] - I_{f, q}(r)\}
\end{align}
So we have $(I_{f, q})^\star(T) \geq  \bb{E}_{\vx \sim q(\vx)}[T(\vx)]$, completing the proof.
\end{proof}
Then we can then substitute $T(\vx)$ with $f'(\exp(r_\psi(\vx)))$, and obtain:
\begin{align}
    \bb{E}_{\vx \sim \pdata(\vx)}[f'(\exp(r_\psi(\vx)))] - 
     (I_{f, q_\phi})^\star(f' \circ \exp \circ r_\psi) \leq \gL_{f-\mathrm{CD}2}(\psi, \phi; \pdata)
\end{align}
where equality holds when $r_\psi(\vx) = 1$ for all $\vx \in \gX$. Therefore, the equilibrium for
\begin{align}
    \min_\phi \max_\psi \gL_{f-\mathrm{CD}2}(\psi, \phi; \pdata)
\end{align}
in which $q_\phi = \pdata$ and $r_\psi(\vx) = 1$, is equal to the equilibrium for 
\begin{align}
    \min_\theta \max_\psi \bb{E}_{\vx \sim \pdata(\vx)}[f'(\exp(r_\psi(\vx)))] - 
     (I_{f, q_\phi})^\star(f' \circ \exp \circ r_\psi)
\end{align}
which is minimization of $D_f(\pdata(\vx) \Vert q_\phi(\vx))$.

\subsection{$f$-CD as Integral Probability Metric Minimization}
If we restrict $r_\psi$ to be selected from $\gF$,  a class of real-valued bounded measurable functions, then $\max_\psi \gL_{f-\mathrm{CD}2}$ corresponds to an IPM between $\pdata$ and $q_\phi$, so the minimax objective can also be treated as minimizing an IPM between $\pdata$ and $q_\phi$.

Compared to using the variational lower bounds of $f$-divergences, $f$-CD:
\begin{itemize}
\item is easy to construct for different types of $f$ (as opposed to the ``tight'' lower bound, which may be hard to compute analytically)
\item has unbiased stochastic estimates that are easy to compute (as opposed to the ``tight'' lower bound, which could lead to biased gradient estimate (MINE))
\end{itemize}
If $\gF$ is not selected properly, the upper bound $\gL_{f-\mathrm{CD}2}$ could be far from the variational lower bound of $f$-divergence between $\pdata$ and $q_\phi$. For a fixed $q_\phi$, the gap is:
\begin{align}
    \sup_{u \in \Delta(q_\phi)}\{\bb{E}_{q_\phi}[f'(\exp(r_\psi(\vx))) u(\vx) - f(u(\vx))]\} - \bb{E}_{q_\phi}[f'(\exp(r_\psi(\vx)))]
\end{align}
which is zero when $r_\psi(\vx) = 0$ for all $\vx \in \gX$. Intuitively, this suggest the use of $r_\psi(\vx)$ functions that are close to zero.

\subsection{More Connections between $f$-Divergence and Dual formulation}
Note that in the maximum likelihood dual form, the $q_\phi$ function tries to approximate the proposed energy (as opposed to the current $f$-CD objective). Moreover, the two objective differ only by a maximum likelihood objective of $q_\phi$, which has a ``constant'' difference with KL divergence. 

Thus, we are interested in finding a form of $f$-CD that links to the MLE dual form more directly.

Consider the following:
\begin{align}
& \gL_{f-\mathrm{CD}2}(\psi, \phi; \pdata) - D_f(\pdata \Vert q_\phi) \\
\leq \ &  \gL_{f-\mathrm{CD}2}(\psi, \phi; \pdata) - (\bb{E}_{\vx \sim \pdata(\vx)}[f'(\exp(r_\psi(\vx)))] - 
     (I_{f, q_\phi})^\star(f' \circ \exp \circ r_\psi)) \\
     = \ & (I_{f, q_\phi})^\star(f' \circ \exp \circ r_\psi) - \bb{E}_{\vx \sim q_\phi(\vx)}[f'(\exp(r_\psi(\vx)))]
\end{align}
where the inequality is from the dual definition of $f$-divergences. We are interested in the local behavior of $q_\phi$ when $r_\psi$ is fixed, i.e.:
\begin{align}
    \nabla_{q_\phi} \left((I_{f, q_\phi})^\star(f' \circ \exp \circ r_\psi) - \bb{E}_{\vx \sim q_\phi(\vx)}[f'(\exp(r_\psi(\vx)))] \right)
\end{align}

First, we need a close form for $(I_{f, q_\phi})^\star(f' \circ \exp \circ r_\psi)$.
\begin{theorem}
Assume that $r_\psi$ satisfies for all $\vx \in \gX$ \js{we do not need this if we make $\Delta(q)$ larger, or simply assume that r is normalized wrt q}:
\begin{align}
    \exp(r_\psi(\vx)) \geq \bb{E}_{q}[\exp(r_\psi(\vx))] - 1
\end{align}
then the optimal $v: \gX \to \bb{R}$ for the following problem
\begin{align}
    \sup_{v \in \Delta(q_\phi)}\{\bb{E}_{q}[f'(\exp(r_\psi(\vx))) v(\vx)] - \bb{E}_{q}[f(v(\vx))]\}
\end{align}
is:
\begin{align}
    v(\vx) = \exp(r_\psi(\vx)) - \bb{E}_{q}[\exp(r_\psi(\vx))] + 1
\end{align}
\end{theorem}
\begin{proof}
We consider the Lagrangian:
\begin{align}
    \bb{E}_{q}[f'(\exp(r_\psi(\vx))) v(\vx)] - \bb{E}_{q}[f(v(\vx))] - \lambda (\bb{E}_q[v(\vx))] - 1)
\end{align}
Taking the functional derivative over $v$ we have:
\begin{align}
    f'(\exp(r_\psi(\vx))) - f'(v(\vx)) = \lambda, \quad \forall x \in \gX
\end{align}
Since $f$ is convex, $f'$ is non-decreasing, so $\forall x \in \gX$, $\exists c \in \bb{R}$ such that
\begin{align}
    \exp(r_\psi(\vx)) - v(\vx) = c
\end{align}
and we obtain $c = \bb{E}_{q}[\exp(r_\psi(\vx))] - 1$ from the fact that $v \in \Delta(q_\phi)$.
\end{proof}
Without loss of generality, we assume that $\bb{E}_{q_\psi}[\exp(r_\psi(\vx))] = 1$, so the corresponding $v(\vx) = \exp(r_\psi(\vx))$. Substitute this into the definition of $(I_{f, q_\phi})^\star(f' \circ \exp \circ r_\psi)$ we have our target gradient:
\begin{align}
  & \nabla_{q_\phi} \left( \bb{E}_{q}[f'(\exp(r_\psi(\vx))) \exp(r_\psi(\vx))] - \bb{E}_{q}[f(\exp(r_\psi(\vx)))] - \bb{E}_{\vx \sim q_\phi(\vx)}[f'(\exp(r_\psi(\vx)))] \right) \\
  = \ & \nabla_{q_\phi} \left( \bb{E}_{q}[f'(\exp(r_\psi(\vx))) (\exp(r_\psi(\vx)) - 1) - f(\exp(r_\psi(\vx)))] \right) \\
  = \ & \nabla_{q_\phi} \left( \bb{E}_{q}[g_f(\exp(r_\psi(\vx)))] \right)
\end{align}
where we define $g_f(u) = f'(u) (u - 1) - f(u)$ for all $u \in \bb{R}^{+}$. Note that $g_f(u)$ is convex for all $f$. 

If we fix $E = \log q_\phi + r_\psi$ (normalized), then the previous term becomes:
\begin{align}
    & \bb{E}_{q}[g_f(\exp(E(\vx)) / q_\phi(\vx))] \\
    \geq \ &  g_f( \bb{E}_{q}[\exp(E(\vx)) / q_\phi(\vx)] ) \\
    = \ & g_f(\int_{\xv \in \gX} \exp(E(\vx)) \mathrm{d}x) = 0
\end{align}
where the equality holds iff. $\exp(E(\vx)) = q_\phi(\vx)$, $\forall \vx \in \gX$.

==> intro.tex <==
% \begin{enumerate}
%     \item Data generation (from $Z_1,Z_2$ to $X$)\\
%     \item Main algorithm
%     \begin{enumerate}
%         \item methods
%         \item pac-bound
%         \item non-overlap support
%         \item Toy experiments
%     \end{enumerate}
%     \item Existence of orthogonal classifier (from $X,w_1$ to $Z_2$)
%         \begin{enumerate}
%         \item definition
%         \item theorem
%     \end{enumerate}
%     \item Use case: Style transfer, domain adaptation
% \end{enumerate}
% Utility: Fairness/DA decompose classifier, intuitively
% Challenge (definition): not well defined, (linear classifier->non-linear). why is not trivial?


Many machine learning applications require explicit control of directions that are orthogonal to a predefined one. For example, to ensure fairness, we can learn a classifier that is orthogonal to sensitive attributes such as gender or race~\citep{Zemel2013LearningFR,Madras2018LearningAF}. Similar, if we transfer images from one style to another, content other than style should remain untouched. Therefore images before and after transfer should align in directions orthogonal to style. Common to these problems is the task of finding an orthogonal classifier. Given any \emph{principal classifier} operating on the basis of \emph{principal variables}, our goal is to find a classifier, termed \emph{orthogonal classifier}, that predicts the label on the basis of \emph{orthogonal variables}, defined formally later.
% To this end, we propose a problem, called \emph{classifier orthogonalization}, whose the goal is to find orthogonal direction to an existing~(principal) classifier \yx{gap: from variable to classifier}. Such a direction is identified by another classifier, termed \emph{orthogonal classifier}. 

The notion of orthogonality is clear in the linear case. Consider a joint distribution where label $Y \sim \gB(0.5)$ and class-conditional distributions are $X|Y=y \sim \gN(\mu_y, I)$ with label dependent means $\mu_0$ and $\mu_1$. If the principal classifier is linear, $w_1=\Pr(Y=1|\theta_1^\top x)$, then the orthogonal classifier $w_2=\Pr(Y=1|\theta_2^\top x)$ must satisfy $\theta_1^\top \theta_2 = 0$, implying orthogonal decision boundaries~(\Figref{img:linear}). Thus the two classifiers $w_1,w_2$ focus on distinct but complementary attributes for predicting the same label. 

Finding the orthogonal classifier is no longer straightforward in the non-linear case. 
% TJ: I would leave this out. It relies on later material to understand
%1) the latent process to generate the data could be non-linear; 2) the classifier that predicts label from data could be non-linear. \yx{For example, when the label-conditioned Gaussians in the above case have different covariances matrices.}
To rigorously define what we mean by the orthogonal classifier, we first introduce the notion of mutually orthogonal random variables that correspond to (conditinally) independent latent variables mapped to observations through diffeomorphism (or bijection if discrete). Each r.v. is predictive of the label but represents complementary information. Indeed, we show that the orthogonal random variable maximizes the conditional mutual information with the label given the principal counterpart, subject to the independence constraint (ensuring complementarity). 

% The classifier orthogonalization 
Our search for the orthogonal classifier can be asked now as follows: given a principal classifier $w_1$ using some unknown principal r.v. for prediction, how do we find its orthogonal classifier $w_2$ relying solely on the orthogonal random variable? The solution to this problem, which we call \emph{classifier orthogonalization}, turns out to be surprisingly simple, making use of an overall classifier $w_x$ in addition to the principal one. We denote the outcome of this orthogonalization process as $w_2=w_x\setminus w_1$.
% perform an abstracted classifier subtraction $w_2=w_x\setminus w_1$. 
The advantage of this construction is that it is based only on the classifiers, not needing to uncover the exact latent mechanism referred to in the definition. 

% Denoting $X$ and $Y$ as the random variables for data and label. In this paper, we focus on the case that $Y$ is discrete. Before introducing orthogonal classifier, we first bring in a notion of orthogonal random variable. Given principal features which is a random variable $Z_1$ defined by a deterministic mapping $z_1$ from the data, \ie $Z_1 = z_1(X)$. Mathematically, our problem is formulated as,
% \begin{align*}
% \max_{Z_2=z_2(X)} I(Z_2; Y \mid Z_1)~~~\text{subject to}~~~I(Z_2;Z_1|Y)=0
% \end{align*}
% % \yx{express the constraint as $I(Z_2;Z_1|Y)=0$?}\hhh{I am fine with it.}
% where $z_2$ is also a deterministic function. We call $Z_1$ is the \emph{principal variable}, $Z_2$ the \emph{orthogonal variable} (to $Z_1$). The \emph{orthogonal classifier} $w_2(x) = \Pr(Y|Z_2=z_2(x))$ takes the orthogonal random variable $z_2(X)$ as inputs when given a \emph{principal classifier} $w_1(x) = \Pr(Y|Z_1=z_1(x))$.

% The classifier orthogonalization problem is abstracted from many real machine learning applications. 
% We want to control our machine learning model to learn itself only in orthogonal directions to a predefined principal direction. For example, in fairness problems, we require our model to be orthogonal to sensitive variables such as gender, race. Another example is partial style transfer, where we aim to change images' style while not touching its content. It requires the discriminator to be orthogonal to the content variable when judging whether two images have the same style.

% Although performing classifier orthogonalization is straightforward in the linear case, it is non-trivial to solve non-linear cases. The non-linearity has two fronts: 1) the mapping from the data to feature could be non-linear; 2) the classifier that predicts label from data could be non-linear. In this paper, we provide conditions that are sufficient for classifier orthogonalization problems to be tractable. We rigorously define the notion of mutually orthogonal random variables through diffeomorphism and independence. We also propose a simple algorithm
% , called \red{\emph{classifier orthogonalization}}, 
% to obtain the orthogonal classifier from the given principal classifier without directly solving the orthogonal learning problem. 


We provide several use cases for the orthogonal classifier, either as a predictor or as a discriminator. As a predictor, the orthogonal classifier predictions are invariant to the \begin{wrapfigure}[14]{r}{0.4\linewidth}
    \vspace{-13pt}
    \centering
    \includegraphics[width=0.7\linewidth]{img/figure_linear.pdf}
    \vspace{-12pt}
    \caption{An illustrative example of orthogonal classifier in a linear case. The dash lines show the decision boundary of principal classifier $w_1$ and orthogonal classifier $w_2$.}
    \label{img:linear}
\end{wrapfigure} principal sensitive r.v., thus ensuring fairness. As a discriminator, the orthogonal classifier enforces a partial alignment of distributions, allowing changes in the principal direction. We demonstrate the value of such discriminator in 1) \emph{controlled style transfer} where the source and target domains differ in multiple aspects, but we only wish to align domain A's style to domain B, leaving other aspects intact; 2) \emph{domain adaptation with label shift} where we align feature distributions between the source and target domains, allowing shifts in label proportions. Our results show that the simple method is on par with the state-of-the-art methods in each task. 


==> src-old/intro-v0.tex <==
% Invariance is an essential concept in physics. It expresses physical principles that govern our universe. For example, the gravity between two objects is invariant to the spatial-temporal coordinates of the objects. Invariance is also be used to describe the principle in human society. For example, we wish people were treated equally no matter what skin color they have. Thus invariance is everywhere as well as cooking machine learning models. The invariance requirement of a machine learning model could naturally stem from the learning target. Take image classification as an example. We instinctively expect the model's prediction to be invariant to understand uncertain transformations of the input image, such as rotation, crop. The invariance constraints could also come from the usage of the model. There are many examples in the field of model fairness. For instance, for a machine learning model that decides whether to loan a client, we hope the model does have a bias on the client's race. 
% However, imposing invariance on a machine learning model is challenging. It is not even clear how to give a proper definition of learning a model with invariance constrain. To start, we consider learning a linear model for the task of binary classification on two-dimensional data. Each data point $x$ has two dimension $x_1,x_2$. We call $x_1$ the \emph{pivot variable} and $x_2$ the \emph{orthogonal variable}. Consider our goal is learning a classifier which invariant to the pivot variable. Further, denoting label by $y$, we define \emph{pivot classifier} $w_1$ being the optimal model that classifies data based on solely pivot variable, \ie $w_1(x_1,x_2)=\Pr(y | x_1)$.
% Similarly, we define \emph{orthogonal classifier} as $w_2(x_1,x_2)=\Pr(y | x_2)$, the optimal classifier that takes orthogonal variable. It is obvious that $w_2$ is our desired model. As shown in \Figref{img:linear}, in the linear case, the pivot classifier $w_1$ and orthogonal classifier $w_2$ are perpendicular to each other. Thus, in the linear case, one could get the orthogonal classifier by finding an orthogonal classifier to the pivot classifier. Such an approach is preferable when directly learning pivot classifier is easier than learning orthogonal classifier, \eg when the pivot variable has much lower dimension than the orthogonal variable.  

% Above, we introduce a new method of constructing a machine learning model invariant to the pivot variable in the context of the linear model for binary classification. In this paper, we extend the methodology to a general machine learning setting. We first mathematically define the pivot/orthogonal variables for any data. We then develop an algorithm to construct the orthogonal classifier from the pivot classifier. Finally, we show that the orthogonal classifier can be used to derive a machine learning model with the desired invariance. For example, in predictive tasks, the orthogonal classifier itself serves as the model with invariance. Simultaneously, in generative tasks, by leveraging the orthogonal classifier, we can learn a generator with certain invariance. To demonstrate the power of our method, we pick three illustrative machine learning tasks: (1)~ \emph{style transfer} where we aim to learn a model that transfers the data from style A to style B while keeping its content invariant during the transformation; (2)~\emph{label shift domain adaptation} where we want a model to align the feature extracted from the source/target domains while keeping the label invariant during the alignment; (3)~\emph{fairness} where we want to a discriminative model that invariant to sensitive variables such as race and gender. Our empirical study shows the utility of building model invariance via the orthogonal classifier. 

==> toy_experiment.tex <==
% \subsection{Evaluation on toy dataset}

% \paragraph{Data generation: } We construct the ColoredMNIST datasets based on the MNIST dataset. The two latents are set to $z_1$=digit color, $z_2$=background color, respectively. \hhh{I feel a something maybe missing here. Since CMNIST image = digit color + background color + digit shape.} We randomly assign a binary label to each datapoint, and pick two digit colors and background colors. Note that there is a one-to-one corresponding between the label and the latents, \eg ``0" $\leftrightarrow$ ``blue digit color” and ``1" $\leftrightarrow$ ``yellow back ground color". For each domain, we define the \textit{bias degree} to be the ratio of the data that obeys this relationship. Those data which don’t follow this relationship are then assigned with random latents. We use the notation $[b_1,b_2]$ to denote the bias degrees on $z_1$ and $z_2$.

% In the following, we assume that we have access to some classifiers on $z_1$, \ie $w_1$. Such classifiers can be obtained by off-the-shelf out-of-distribution generalization algorithms, such as IRM and TRM trained on several environments. Our goal is to classify data on the $z_2$ direction.
% \paragraph{Architecture: } We used a 4-layer CNN. SGD with learning rate $0.1$ and weight decay $1e-4$ acts as the optimizer.

% \paragraph{Baselines: } \textbf{(i) Oracle:} Classifiers that only uses $z_2$ for prediction. We train the oracle classifier on the bias degrees $[0,0.6]$, \ie only $z_2$ is correlated with the label.



% % \begin{align*}
% %     \textrm{Var}(\E_{\hat{P}_1\hat{P}_2}[\frac{1-w_1}{w_1}\log(w_2)]) &= \textrm{Var}\left(\frac{1}{n}\sum_{i=1}^n\frac{1-w_1(f(z_1^i,z_2^i))}{w_1(f(z_1^i,z_2^i))}\log(w_2(f(z_1^i,z_2^i)))\right)\\
% %     &=\textrm{Var}\left(\frac{1}{n}\sum_{i=1}^n\frac{Q_1(z_1^i)}{P_1(z_1^i)}\log(w_2(f(z_1^i,z_2^i)))\right)\\
% %     &=\frac{1}{n}\int P_1(z_1)P_2(z_2)(\frac{Q_1(z_1)}{P_1(z_1)}\log w_2(f(z_1,z_2)))^2 \rvd z_1\rvd z_2- \frac{1}{n}\mu^2\\
% %     &=\frac{1}{n}\int \frac{({Q_1(z_1)P_2(z_2)}\log w_2(f(z_1,z_2)))^2}{P_1(z_1)P_2(z_2)} \rvd z_1\rvd  z_2- \frac{1}{n}\mu^2 \\
% %     &= \frac{1}{n}\int \frac{Q_1^2(z_1)}{P_1(z_1)}\rvd z_1\int {P_2(z_2)(\log w_2(f(z_1,z_2)))^2} \rvd  z_2- \frac{1}{n}\mu^2\numberthis \label{eq:var_reweight}
% % \end{align*}

% In contrast, the variances of mini-batch objective of $w_x$ and $w_1$ are irrelevant to the density ratio $\frac{Q_1}{P_1}$. The influence of the $ \frac{Q_1^2(z_1)}{P_1(z_1)}\rvd z_1$ term:


